Network Agile Preference-Based Prefetching for Mobile Devices

For mobile devices, communication via cellular networks consumes more energy, and has a lower data rate than WiFi networks, and suffers an expensive limited data plan. However the WiFi network coverage range and density are smaller than those of the cellular networks. In this work, we present a behavior-aware and preference-based approach to prefetch news webpages that a user will be interested in and access, by exploiting the WiFi network connections to reduce the energy and monetary cost. In our solution, we first design an efficient preference learning algorithm based on keywords and URLs visited, which will keep track of the user's changing interests. By predicting the appearance and durations of the WiFi network connections, our prefetch approach then optimizes when to prefetch what webpages to maximize the user experience while lowing the prefetch cost. Our prefetch approach exploits the idle period of WiFi connections to reduce the tail-energy consumption. We implement our approach in iPhone. Our extensive evaluations show that our system achieves about 60% hit ratio, saves about 50% cellular data usage, and reduces the energy cost by 9%.

==> abstract.tex <==
For mobile devices, communication via cellular networks consumes more
 energy, and has a lower data rate than WiFi networks,
 and suffers an expensive limited data plan.
However the WiFi network coverage range and density are smaller
 than those of the  cellular networks.
In this work, we present a behavior-aware and
 preference-based  approach to  prefetch  news webpages
 that a user will be interested in and access, by 
  exploiting the WiFi network connections to
 reduce the energy and monetary cost.
In our solution, we first design
  an efficient preference learning algorithm based  on
 keywords and URLs visited,   which will keep track of the
 user's changing interests.
By predicting the appearance and durations of the WiFi network
 connections, our prefetch approach then optimizes when to prefetch
 what webpages to maximize the user experience while lowing the
 prefetch cost.
Our prefetch approach exploits the idle period of WiFi connections to
reduce the tail-energy consumption.
We implement our approach in iPhone.
Our extensive evaluations show that  our system achieves about $60\%$ hit
 ratio, saves about  $50\%$ cellular data usage, and reduces the energy
 cost by $9\%$.


==> conclusion-new.tex <==
In this paper we designed a network-agile preference-based prefetching method for mobile devices.
We implemented our method in iPhone and conducted extensive evaluations on the performances of our methods.
Our evaluations show that our prefetching based approach is able to reduce the cellular network access by about $50\%$ 
 and reduce the energy cost by about $9\%$.
 


==> intro-new.tex <==

According to a recent study \cite{webusagekim2011}, mobile web
browsing is growing significantly and expected to surpass the desktop
web browsing by 2015.Web browsing and news reading
 account for a large proportion of the time and data used by smartphones.
Smartphone users with a data plan spend
on average 300 minutes per month browsing the web, which is comparable
to mobile voice usage~\cite{applicationcap}.
The global smartphone
study run by Zokem shows that web browser is the single most popular
data application which accounts for 54\% of data application face time and 50\% of data
volume for smartphones \cite{applicationcap}.
%and the users read news for most of the time when they use web
%browser \cite{enhancingyu2011} .
%Accessing maps and directions is the no. 1 mobile activity (81\%),
%followed by three media-related activities: social networking (76\%)
%accessing local information (73\%) and reading news (68\%).
Among the user's web browsing activities, reading news makes up for 68\% of the time which is one of the most frequent
activities~\cite{adobe}.


Typically there are two different networking access approaches:
 cellular network and WiFi network.
Although the cellular network is almost ubiquitous and its
 coverage seems not to be a problem, the limited data plan, higher price,
 lower data rate and more energy consumption
 \cite{lehr2003wireless,balasubramanian2009energy} make the smartphone
 users  prefer using the WiFi network whenever possible.
It is thus natural to switch to WiFi network access whenever possible.
Seamless switch between networks has been proposed to improve the
networking performances
\cite{chakravorty2004performance,niyato2007wireless}.
To further reduce the energy and monetary cost while not sacrificing the
 user experience,
 in this work we present a seamless transparent solution that
 automatically prefetches contents and switches between networks.
Techniques of prefetching contents \cite{fan1999web,jiang1998web}
 and seamlessly switching networks
 \cite{chakravorty2004performance,niyato2007wireless}
 have been  used previously to address various challenges.
To make the content prefetching work for mobile devices, a number of
 challenges must be addressed.
In general, we need to know when to prefetch what contents such that
the user experience is not deteriorated and the overall  energy cost
and monetary cost for data plan is reduced.
Then we need to  learn and predict the availability of WiFi network
 access and the user web-browsing preference.

To address the challenge of knowing what to prefetch, we  predict what
 webpages the  user will visit in the near future and prefetch them via WiFi
 network at an appropriate time.
When the user indeed wants to read these webpages later,
 there is no need to access them via cellular network.
With the advances in mobile devices, the memory is getting larger and
 computation capacity are becoming stronger, so it is possible for
 mobile devices to learn the user's preference and prefetch the
 web pages in advance.
Most of the previous work on web prefetch is based on the URLs of web
 pages visited by the user in the past.
Moreover, the majority techniques for web prefetch focus on
 short-term prefetching, where the webpages will be visited in a short
 time period, \eg, a few seconds to a few minutes at most.
The short-term  prefetch technology can be divided into two
categories: probability-based and clustering-based approach.
In probability-based approach, the web request sequence is assumed to
 follow a certain probability distribution and the future request
 hence can be anticipated according to the pattern. For the clustering
 based approach, the decision is based  on the assumption that the webpages close to the previous downloaded webpages are more likely
 to be accessed in the future.

In this paper we focus on the long-term web prefetch  which
prefetch the web contents much earlier (\eg, half an hour to several hours)
before the user browses the webpages.
An motivating example for this long-term prefetch
  is as  follows.
Assume that a user Bob goes to work at 8:00 am in the morning by
 train and he is used to read news on his way to the office.
Assume there is no WiFi network in the train and Bob has a WiFi
network at home.
By profiling the news types and frequently visited pages by Bob in the
train, we can prefetch these dynamic contents for Bob when he is about
to leave home for work.
Although contents prefetched might be obsolete or be invalided in the
future, we assume that the user's experience will not drop by reading
the news prefetched about an hour ago.


Unfortunately, for news prefetch, URL-based approach is  insufficient
 because each piece of news is often assigned a unique URL
 and a user seldom reads the same news  twice.
It is hard to predict what kind of news a user will be interested in
 purely based on the URL of the news.
In this work, we  present a prefetching approach that combines the
 keyword-based and URL-based approach.
Based on the list of most visited websites and sections by the users (\eg, cnn.com,
 cnn.com/World), we  assign different weights to different websites and  sections.
We also capture the user's dynamic preference on news by assigning
 decayed weights to the list of mostly appeared keywords in the news.
We then sort the list of possible news based on
 a combination of the websites' weights and keywords weights.
This will give us a list of news to prefetch.

The second challenge is to decide when to prefetch these contents.
Several challenges make the decision of prefetch timing difficult:
 (1) if a user has a WiFi network access now, we need to predict when the
  user will move outside the coverage region of the WiFi networks;
 (2) even if we know when the WiFi network connection will be lost, we
 need to estimate the time needed for prefetching the contents so that
 the prefetched contents are mostly up-to-date when the user reads it;
(3) the prefetching activities should not interfere the regular
 network usage activities by the user (otherwise, the user experience
 will be deteriorated).

In summary the main contributions of this work are as follows.
We combine the keyword-based and URL-based prefetching approach to
predict the webpage a user will be interested in.
We also present a network condition prediction approach
 that can start contents prefetch automatically.
In addition, we propose a prefetch scheduling algorithm to exploit
 idle time of the network to prefetch the web pages.
See Section~\ref{sec:design} for details of our system design and approaches.
We implement the  prototype system in iPhone and conduct extensive
 evaluations on the performance of our system.
The experimental results reported in Section \ref{sec:evaluation}
show that our system has high hit ratio
 and low waste ratio while at the same time is energy efficiency and data
 saving.





==> problem.tex <==

\subsection{Problem Formulation}

Given the user's access history and the past network condition,
we want to prefetch the web pages via WiFi network for the user to
browse when the WiFi network is not available.
Here we focus on prefetching  news web page from news
 websites.
To capture the user behaviors and for easy manipulation, we designed and
 implemented a web browser for iOS.
We assume that the  user visits web pages through our browser
 and we can keep track of the user's access history.
In addition, to keep the prefetching activities transparent from the
 end-users while not interfering the regular browsing activities of
 end-users, our system  should prefetch the webpages automatically by
 carefully exploiting the idle network connections.
Our system also will predict the network connections, especially, when
 the end-user will have a WiFi network access and when the end-user
 will leave the current WiFi network.
Based on this network prediction and the user browsing behavior and
 preference model, we should carefully schedule  the prefetching jobs
 such that we can prefetch the most latest related news before the
 user leaves the current WiFi network coverage.
Observe that a user still needs to use cellular network connections
 when the user wants to read some news webpages not yet prefetched.
An intermediate goal here is to reduce such cellular network connections as much
 as possible.
The ultimate goal is to carefully decide what contents to be
 prefetched at what time such that the overall energy consumption and
 the paid network access are reduced.

\subsection{Challenges and Approaches}

%\subsubsection{Data Issue}
%Not only the energy cost but also the data cost is a concern for our
%design. As the data plan is always limited and relatively more
%expensive than the WiFi network, the data cost also need to be taken
%into consideration. Though several carrier provide unlimited data, it
%is not unlimited. If the user's data usage surpass certain
%limit,  the speed will be decreased, which makes it will take two or
%three minutes to open a web page. If we can prefetch the news via
%WiFi connection which is almost free, then data cost can be saved as
%the contents is already fetched into the mobile device via WiFi
%network in advance.

%It is possible that the prefetching will cost more energy than fetch
%it via cellular network, so it seems that it is better not to
%prefetch the content. Though it is not worth to prefetching
%considering the energy consumption, it is still meaningful to
%prefetch the content if the data usage will decrease. So we need to
%estimate both the energy and data cost to decide what to prefetch and
%how much to prefetch.

\subsubsection{News Preference Issue}

How to learn the user's preference is a challenging  problem.
Learning the preference by the URLs visited
 by the user is not accurate for news prefetching, as a user
 always read the newly added news which often have  new URLs, which are
 hard to predict.
Another technique for learning the user's preference is to perform
 statistics (\eg, the keywords frequencies
 \cite{embley1999conceptual}) on the news webpages
 visited by the user.
Keywords extraction has been widely used for understanding webpages
\cite{yih2006finding,embley1999conceptual}.
Unfortunately these techniques cannot be directly applied here as our
 goal is to reduce energy consumption and data access:
 If we analyze the whole news word by word, it will cost a
 large amount of energy and might not find the keywords in which the
 user are really interested.
Besides, the keyword list maintaining is also challenging since the
 keyword list will keep growing as the time goes on and some
 keywords will become obsolete.
We need to refresh the keywords list such that the keyword list size
 is bounded and it indeed actually captures the user's recent interests.

Not only the keywords, the visit paths within a news website are also
 important for preference learning.
It will consume a large amount of
 time to search the news from all news websites.
Even for the same website, there exits always multiple
 sections for different categories and searching all the sections also
 costs time.
Thus the prefetching  need to combine the keywords and the
 visit path of the websites, that is we need to prefetch the news
 including the keywords from the user's favorite websites.
Instead of keep tracking all the visited URLs, we only keep track the
 URLs of the  news website and the URLs of the sections and subsections
 in the news website (see Fig.~\ref{fig:website} for details).

\subsubsection{Performance Issue}

Performance is a major concern due to the limited bandwidth of the
 mobile device.
Fast loading of a webpage is what the user
 desires, so the prefetching is supposed not to interfere the
 user's normal browsing.
It is  better that we prefetch contents when there
 are no regular networking activities:
 prefetching should be interleaved  among regular  data transferring.
In order to exploit the period after the data
 transferring is completed, we need to estimate when the next regular web
 browsing requests will occur and how long a prefetching job will take.
Observe that a user often experiences various networking speeds due to
 different networking environment (\eg, time, location, and APs).
However, our extensive evaluations (downloading more than $300$
 webpages) at three different locations show that the fetch times for
 webpages do not have a large variance.
For simplicity, in this work, we will use the mean fetch time as the
 estimated time for prefetching any new webpage.

\subsubsection{Energy Issue}

Due to the limited lifetime of the battery in mobile devices, energy
 consumption is an important consideration for the mobile prefetching
 approach.
Prefetching web pages will consume large amount of energy
 when using wireless connection, especially when using cellular
 network or the connection is poor.
WiFi networks, in general, consume less
 energy than cellular network,
 so if we can always prefetch contents via WiFi network it will save
 the energy consumption.
However, the WiFi network is not always available for some areas.
Thus, we should exploit the WiFi connections whenever possible.
To ensure that the prefetched news is up-to-date, we will delay the
 prefetch as late as possible.

Though the WiFi network is energy saving compared to the cellular
 network, both WiFi and cellular network waste some energy when the
 data transfer is completed, which is called "tail energy"
 \cite{tailtheft,energymobile}.
Since the  mobile device is at high powering setting when transferring
 data via  WiFi or cellular network, after the mobile device completes
 the transferring it still consumes more energy than normal setting.
Though the "tail energy" is unavoidable for the mobile devices,  we
 can also exploit the period after the transferring to prefetch the news
 for the user in advance, such that the tail energy will not be wasted.
%We will exploit the interval between two web requests to prefetch the
% web pages such that  the prefetching will not interfere the
% user's web browsing.
%This also helps to reduce the "tail energy".
Thus we also need to learn the user's behavior such as
 how long the user stays in the current WiFi network
 and the time separation between two normal consecutive networking
 activities.

On the other hand, prefetching the useless news that the user
 will not read in the future also wastes a certain amount of energy.
If the news is with low possibility to be read in the future, then it is
 better  not to prefetch it, instead let the user access it via
 cellular  network  when needed.
Though the more we prefetch, the higher possibility we
 prefetch all the contents to be accessed,
 but the more energy consumption.
Thus we need to balance the amount of the news to prefetch and
accuracy of the prefetching.





==> related.tex <==

\subsection{Desktop Prefetch}
Web prefetching has been studied for a long time. The primary
objective of prefetching technique in desktop computer is to reduce
the latency of web page loading and increase the hit ratio of the
prefetched web pages.

\subsubsection{Short-Term Prefetching}
Short-term prefetching technique aims at  predicting the web pages to
be visited  in the near future say the next one or two web
pages. Markov model is an important approach for short-term
prefetching. The Markov-based prefetching technique predicts the next
web pages to be visited by  analyzing the past visit
sequence. Xing~\cite{newmarkov} proposed a hybrid-order tree-like
Markov model that can predict web access precisely.
By analyzing the user's visit path,  Jin~\cite{hiddenmarkov}
proposed  a prefetching model based on the Hidden Markov Model (HMM)
that is able to capture and mine the user's information
requirement for the  future  and then makes semantic-based prefetching
decisions.

Firefox~\cite{firefox} introduced a new strategy for website
optimization:  link prefetching. The browser can prefetch specified
web pages based on the prefetching hints provided by the web page.
It utilizes browser idle time to download or prefetch documents that
the user might visit in the near future.
In HTML5~\cite{html5} prefetching is done via the LINK tag, specifying
"prefetch" as the \textit{rel} and the \textit{href} being the path to the document.

\subsubsection{Long-Term Prefetching}

In contrast to the short-term prefetching, long-term
 prefetching uses long-term steady state object access rates and update
 frequencies to make prefetch decisions.
Markatos~\cite{topten1998} proposed a top 10 approach for
 prefetching: the server keeps the most popular
 documents requested by the proxies and the clients, and then these top
 10 documents will be considered for prefetching by the
 clients.
In the approach by Shin~\cite{domaintop},  the proxy calculates both
 the most  popular domains and most popular documents in those domains, then
 prepares a rank list for prefetching.
Keyword-based prefetching for Internet news services is presented
 in~\cite{keyword2002} \cite{semanticbased}.
The keyword-based approach is able to prefetch the URLs that is rarely accessed or have never been before.
%Using the Zipf-like \cite{zipf1949} access patterns of the web,
% techniques were proposed to improve the hit ratio.
Venkataramani \etal~\cite{longterm2001} presented and evaluated a long term
 prefetching policy based on both object request rates and lifetimes.
Wu~\cite{objectiveopt} proposed a H/B-Greedy prefetching  to
 improve the H/B metric which combines
 the effect of increasing hit rate (H) and reducing the extra bandwidth
 (B) consumed by prefetching.

\subsection{Mobile Prefetch}

The prefetching technique for mobile device also needs to be energy
 and data efficient.
Balasubramanian~\cite{energymobile} presented a measurement study of
the energy consumption characteristics of three widespread mobile
networking technologies and finds that 3G and GSM incur a high tail
energy overhead incurred by staying in high power states after
completing a transfer.
Liu \etal~\cite{tailtheft} proposed the TailTheft to schedule a number of
transmissions to the Tail Time of other transmissions.
Balasubramanian~\cite{augment3g} explored the use of
 intermittently available WiFi to reduce 3G data usage and ease
 pressure on cellular networks.
\cite{poweraware} proposed the VAP scheme which can
 dynamically adjust the number of prefetch  jobs based on the current
 energy level to prolong the system running
 time.
\cite{prefetchinmobile} described a  prefetch
 scheme that adapts to different network systems.
\cite{informed2012} presented a
 cost-benefit analysis to decide when to prefetch based on the
performance such as latency reduction, the cost of energy and monetary
cost or data usage.
%They put the three concerns: performance, energy
%usage, data consumption together to make the prefetch decision.


Lymberopoulos~\cite{pocket2012} presented a prefetching technique based
 on machine learning approach for mobile phone.
Their prefetch technique is based on the visited URLs and only focus
 on the URLs  visited most frequently.
They extract spatiotemporal feature form the user's browsing
 behavior and use these features for training.
Their approach also decreases the energy
 consumption by offloading the machine leaning job to the remote
 server.
Song~\cite{cachemiss} proposed novel algorithms to mine the
 association rules and use them to construct the prefetch sets and
 proposed a cache-miss-initiated prefetch (CMIP) scheme to reduce
 system resources consumption such as bandwidth and power.
Armstrong~\cite{dynamicupdate}  employs a pair of proxies, located on the mobile client and on a fully-connected edge server respectively. 
%to minimize the battery consumption caused by wireless data transfers to and from the mobile device. 
The client specifies her interest by highlighting portions of already fetched webpages through the browser.  If relevant changes have occurred, the edge proxy will aggregate the updates as one batch to be sent to the client. 
%The proxy running on the mobile device can pull these updates from the edge proxy, either on-demand or periodically, or can listen for pushed updates initiated by the edge proxy.
 Komninos~\cite{calendar} presents a prefetching approach based on the contextual information regarding the user's activities and interests extracting from their electronic calendar.

To enhance the prefetching performance, it is also important to predict the
network environment \cite{hotspot}.
Higgins~\cite{informed2012} presented a
 predictive frame for mobility-aware prefetching.
It uses the Gauss-Markov model to estimate the movement and further
 estimate the  probability of the future location.




